Skeleon-Based Typing Style Learning For Person Identification

We present a novel architecture for person identification based on typing-style, constructed of adaptive non-local spatio-temporal graph convolutional network. Since type style dynamics convey meaningful information that can be useful for person identification, we extract the joints positions and then learn their movements' dynamics. Our non-local approach increases our model's robustness to noisy input data while analyzing joints locations instead of RGB data provides remarkable robustness to alternating environmental conditions, e.g., lighting, noise, etc. We further present two new datasets for typing style based person identification task and extensive evaluation that displays our model's superior discriminative and generalization abilities, when compared with state-of-the-art skeleton-based models.

==> Figures/figure1.tex <==
\begin{figure}[t]
\begin{center}
  \includegraphics[width=\linewidth]{Figures/Images/Dataset_wide.png}
\end{center}
  \caption{Frames from 60Typing10 dataset. Who is who? It is easy to tell the difference between people when there are only 6 of them, but what happens when there are 60? A single image has its limitations since it only contains visual information. Video, on the other hand, contains a temporal dimension that provides new information regarding the person's dynamic. In this work, we present a model that learns to classify people according to their unique dynamic with remarkable accuracy.}
\label{fig:dataset_example}
\end{figure}

==> Figures/figure7.tex <==
\begin{figure*}
\centering  
\subfigure[AGCN $\nth{1}$ subset,Bones]{\includegraphics[width=0.3\linewidth]{Figures/Images/AGCN_PA1_Bones.png}}
\subfigure[AGCN $\nth{2}$ subset, Bones]{\includegraphics[width=0.3\linewidth]{Figures/Images/AGCN_PA2_Bones.png}}
\subfigure[AGCN $\nth{3}$ subset, Bones]{\includegraphics[width=0.3\linewidth]{Figures/Images/AGCN_PA3_Bones.png}}
\subfigure[ANLGCN $\nth{1}$ subset, Bones]{\includegraphics[width=0.3\linewidth]{Figures/Images/ANLGCN_PA1_Bones.png}}
\subfigure[ANLGCN $\nth{2}$ subset, Bones]{\includegraphics[width=0.3\linewidth]{Figures/Images/ANLGCN_PA2_Bones.png}}
\subfigure[ANLGCN $\nth{3}$ subset, Bones]{\includegraphics[width=0.3\linewidth]{Figures/Images/ANLGCN_PA3_Bones.png}}
\subfigure[AGCN $\nth{1}$ subset, Joints]{\includegraphics[width=0.3\linewidth]{Figures/Images/AGCN_PA1_Joints.png}}
\subfigure[AGCN $\nth{2}$ subset, Joints]{\includegraphics[width=0.3\linewidth]{Figures/Images/AGCN_PA2_Joints.png}}
\subfigure[AGCN $\nth{3}$ subset, Joints]{\includegraphics[width=0.3\linewidth]{Figures/Images/AGCN_PA3_Joints.png}}
\subfigure[ANLGCN $\nth{1}$ subset, Joints]{\includegraphics[width=0.3\linewidth]{Figures/Images/ANLGCN_PA1_Joints.png}}
\subfigure[ANLGCN $\nth{2}$ subset, Joints]{\includegraphics[width=0.3\linewidth]{Figures/Images/ANLGCN_PA2_Joints.png}}
\subfigure[ANLGCN $\nth{3}$ subset, Joints]{\includegraphics[width=0.3\linewidth]{Figures/Images/ANLGCN_PA3_Joints.png}}
\caption{Learned adjacency matrices of ANLGCN and AGCN from all subsets and both streams. While all matrices learn new dependencies, ANLGCN matrices are less organized and binary. Therefore, their information is more abundant, and they able to realize less trivial dependencies that neglected in the AGCN matrices.}\label{Learned_adj}
\end{figure*}

==> Tables/Table2.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{l c}
Model & Acc(\%)\\
\hline
HCN~\cite{HCN} & 94.18\\
STGCN~\cite{GCN3} & 93.59\\
3sARGCN~\cite{ARGCN} & 91.08\\
PBGCN~\cite{PBGCN} & 95.98\\
2sAGCN~\cite{2sGCN} & 96.88\\ 
\hline
StyleNet & \textbf{99.57}\\
\hline   
\end{tabular}
\end{center}
\caption{Test accuracy of user classification on unseen sentence experiment on~\textit{80Typing2} dataset. Each model trained on 1 sentence and tested on the other sentence that did not appear in training.}
\label{80Tab1}
\end{table}

==> Tables/Table3.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|}
Model & Acc(\%)\\
\hline
HCN~\cite{HCN} & 99.66\\
STGCN~\cite{GCN3} & 99.64\\
3sARGCN~\cite{ARGCN} & 99.44\\
PBGCN~\cite{PBGCN} & 99.84\\
2sAGCN~\cite{2sGCN} & 99.85\\ 
\hline
StyleNet & \textbf{99.98}\\
\hline 
\end{tabular}
\end{center}
\caption{Test accuracy of user classification on seen sentences experiment on~\textit{80Typing2}. The training set includes five repetitions from both sentences, while the validation set includes one repetition from both sentences, and the test set includes four remaining repetitions from both sentences.}
\label{Tabreid}
\end{table}
